LAMP: Prompt Layer 7 Attack Mitigation with Programmable Data Planes

While there are various methods to detect application layer attacks or intrusion attempts on an individual end host, it is not efficient to provide all end hosts in the network with heavy-duty defense systems or software firewalls. In this work, we leverage a new concept of programmable data planes, to directly react on alerts raised by a victim and prevent further attacks on the whole network by blocking the attack at the network edge. We call our design LAMP, Layer 7 Attack Mitigation with Programmable data planes. We implemented LAMP using the P4 data plane programming language and evaluated its effectiveness and efficiency in the Behavioral Model (bmv2) environment.

==> Makefile <==
PRJ = aggregate

# to use eps figures
DVIOPT = -P cmz -t letter -G0

all : viewpdf 

#${PRJ}.dvi : *.tex *.bib 
#	pdflatex ${PRJ}; bibtex ${PRJ}; pdflatex ${PRJ}; pdflatex ${PRJ} 
#
#${PRJ}.ps : ${PRJ}.dvi
#	dvips ${DVIOPT} -o ${PRJ}.ps ${PRJ}.dvi

#${PRJ}.pdf : ${PRJ}.ps
${PRJ}.pdf : *.tex *.bib 
	pdflatex ${PRJ}; bibtex ${PRJ}; pdflatex ${PRJ}; pdflatex ${PRJ} 
#	ps2pdf ${PRJ}.ps ${PRJ}.pdf

dvi : ${PRJ}.dvi

ps : ${PRJ}.ps

pdf : ${PRJ}.pdf

viewdvi : ${PRJ}.dvi
	xdvi ${PRJ}.dvi &

viewps : ${PRJ}.ps
	open ${PRJ}.ps &

viewpdf : ${PRJ}.pdf
	open ${PRJ}.pdf &

# to use non-eps figures.
#all : view 

#${PRJ}.pdf : *.tex 
#	pdflatex ${PRJ}; bibtex ${PRJ}; pdflatex ${PRJ}; pdflatex ${PRJ}

#pdf: ${PRJ}.pdf

#view : ${PRJ}.pdf
#	open ${PRJ}.pdf &

pack : pdf
	/bin/rm -f ../${PRJ}.tgz; tar -zcf ../${PRJ}.tgz Makefile *.tex IEEEtran.cls net.bib ${PRJ}.pdf figure 

clean:
	/bin/rm -f *.toc *.aux *.bbl *.blg *.log *.dvi *~* *.bak ${PRJ}.pdf ${PRJ}.ps

distclean:
	/bin/rm -f *.toc *.aux *.bbl *.blg *.log ${PRJ}.dvi ${PRJ}.ps ${PRJ}.pdf *~* *.bak

#cut : ${PRJ}.dvi 
#	dvips -t letter -o summary.ps -p=2 -l=2 ${PRJ}.dvi
#	ps2pdf summary.ps summary.pdf
#	/bin/rm summary.ps \
#
#	dvips -t letter -o description.ps -p=3 -l=17 ${PRJ}.dvi
#	ps2pdf description.ps description.pdf
#	/bin/rm description.ps \
#
#	dvips -t letter -o references.ps -p=18 -l=20 ${PRJ}.dvi
#	ps2pdf references.ps references.pdf
#	/bin/rm references.ps



==> bg.tex <==
% \section{Background}
%\label{bg}
%\subsection{Attacks on the application layer}
%Layer 7 attacks, such as application layer DDOS attacks, are directed against the applications and resources of a network, e.g., a web-server, database, CPU and disk. They also may target application layer protocols, such as HTTP, FTP, SSH. Usually, these attacks are initiated from a certain control center and conducted within several stages, including (1) Network scanning, e.g., random dictionary attacks against end hosts of a network, in order to gain an administrative control over vulnerable devices;  (2) Recruiting them into botnets; (3) Running a coordinated attack against the victim(s) using a botnet~\cite{kolias2017ddos}. 
%Another example of the Layer 7 attack with the centralized control center are crypto ransomware attacks~\cite{orman2016evil}.

%Note, that for every stage an attacker needs to use a legitimate source IP address for its control center. On one hand, this disables a common attack detection technique, that verifies the correctness of the source IP address of each packet~\cite{prabha2010mitigation}. On the other hand, if an attack was detected on time (for example, by one of the scanned hosts), it can be blocked using a simple drop rule for the attacker's IP address. We employ this property in LAMP to design fast mitigation technique for preventing development of a Layer 7 attack at its earliest stage.

%to add: encryption attacks?

\section{Protocol Independent Switch Architecture and P4}
% PISA concept: what it does
% P4 lanugage: what it can do
% LAMP implementation in P4
The emergence of various types of cloud services, data centers, advent of the Internet of Things (IoT) and the increasing demand for them requires revision of computer networking fundamentals, for example, modification of the current networking protocols and designing new protocols. Software Defined Networking (SDN) has been an important step towards vendor-independent and flexible computer networking. However, the fixed configuration of the data plane has been a constraint for generating and implementing some of the new ideas that involve novel protocols, new header-types and different behavior of the ingress and egress pipelines~\cite{p4vssdn}. Protocol Independent Switch Architecture and P4 language~\cite{bosshart2014p4} have removed above-mentioned restrictions on the data plane. In this work, we use P4 to change the structure of the ingress packets in order to track their path inside a network. In addition, we design a new protocol for alert messages, that are derived from the attacked host and eventually received by an ingress edge switch of the malicious network traffic. P4 enables us to implement this functionality without northbound traffic towards the control plane or controller, which often represents an attractive target for hackers~\cite{sezer2013we}.

==> bg.tex_old.tex <==
\section{The equivalence of forwarding tables problem}
\label{sec:bg}
We begin to consider the problem of the equivalence of forwarding tables by giving the formal definitions.
\begin{defn}Suppose there is a forwarding table $T$, which consists of entries $p^{1}, p^{2}, .., p^{n}$, where $p^{i} = \{0, 1\}^{l_{i}}$, where $l_{i}$ is the length of the entry $p^{i}, {i}\leq{n}$. Also there is a string $s = \{0, 1\}^{l_{s}}$. We can denote $p^{i}$ as $p_{1}p_{2}..p_{l_{i}}$ and $s$ as $s_{1}s_{2}..s_{l_{s}}$.
	\\ Then, $p^{i}$ is a \textbf{\textit{Longest Prefix Match}} for $s$ in $T$ (or $p^{i} = LPM_{s}(T)$), if
	\begin{enumerate}
		\item $l_{i} \leq l_{s}$
		\item $p^{i}$ is a Prefix for $s$ (or $p_{1} = s_{1}, p_{2} = s_{2}, .. , p_{l_{i}} = s_{l_{i}}$).
		\item $\nexists p^{j} = \{0, 1\}^{l_{j}}: p^{j}$ is a Prefix for $s$ and $l_{j} > l_{i}$.
	\end{enumerate}
\end{defn}
In the following definitions we denote the value of next hop for a prefix $p$ in the table $T$ as $nexthop_{T}(p)$.
\begin{defn}The forwarding tables $T_{1}, T_{2}, ..., T_{m}$ are \textbf{\textit{equivalent}}, if and only if, for every possible IP address $\omega = \{0,1\}^{n}$,  $nexthop_{T_{1}}(LPM_{\omega}(T_{1})) = nexthop_{T_{2}}(LPM_{\omega}(T_{2}))= ... = nexthop_{T_{m}}(LPM_{\omega}(T_{m}))$. $n$ is the fixed length of the IP address.
\end{defn}
According the definition above, to verify the equivalence of forwarding tables requires $2^{32}$ or $2^{128}$ depending on the format of forwarding tables (IPv4 of IPv6).  Our goal is to draw an equivalent definition with a feasible number of the required steps. To do that, we prove the property of the \textit{Joint Forwarding Table}, combined by entries of the comparable tables.
\begin{theorem}
		Let $T$ be a union of two routing tables $T_{1}, T_{2}, ..., T_{m}$. Then, $\forall \omega = \{0,1\}^{n}, LPM_{\omega}(T_{i}) = LPM_{p}(T_{i})$, where $p = LPM_{\omega}(T)$ and $i = 1, 2, ..., m$.
		\begin{proof}
			Let's denote entry $p$ as $p_{1}p_{2}..p_{l}$, its length $l\leq n$ and $\omega$ as $\omega_{1}\omega_{2}..\omega_{n}$. If $p = LPM_{\omega}(T)$, then $\omega = p_{1}p_{2}...p_{l}\omega_{l}\omega_{l+1}..\omega_{n}$. 
			\\ Suppose, $LPM_{p_{1}p_{2}...p_{l}\omega_{l}\omega_{l+1}..\omega_{n}}(T_{i}) \neq LPM_{p_{1}p_{2}..p_{l}}(T_{i})$. It is possible only if there is an entry $p^{'}$ in the routing table  $T_{i}$ such as its length $l < l^{'} \leq n$, and that entry is a Prefix for $w$. But then, that entry exists in $T$ and $p$ cannot be a \textbf{Longest Prefix Match} for $\omega$ and $T$. Thus there is a contradiction with the hypotheses of the theorem that $p = LPM_{\omega}(T)$.
		\end{proof}
\end{theorem} 
Let's then rewrite the Definition 2 according to the Theorem 1.
\begin{defn}The forwarding tables $T_{1}, T_{2}, ..., T_{m}$ are \textbf{\textit{equivalent}}, if and only if, $\forall \omega = \{0,1\}^{n}$,  $\forall p = LPM_{\omega}(T),$ where $T$ is the union of $T_{1}, T_{2}, ..., T_{m}, nexthop_{T_{1}}(LPM_{p}(T_{1})) = nexthop_{T_{2}}(LPM_{p}(T_{2})) = ... = nexthop_{T_{m}}(LPM_{p}(T_{m}))$. 
\end{defn}
Although the new definition still refers the scope of IP addresses $\omega$, the set of \textit{Longest Prefix Matches} in $T$ is bounded by the number of entries in $T$ and can be defined regardless to $\omega$. We discuss it in the next section.


==> intro.tex_old.tex <==
\section{Introduction}
\label{sec:intro}
The Internet architecture divides the global network into Autonomous Systems (ASes). Every AS is assigned with unique Autonomous System Number (ASN), and a block of IP addresses - IP prefixes. For example, the IP prefix 92.65.64.0/24 represents the block of $2^{8}$ IP addresses with first 3 octets equal to 92, 65 and 64. The assignment of IP blocks and ASNs is regulated by Internet Assigned Numbers Authority (IANA). The routing within ASes is handled by Interior Gateway Protocols, such as OSPF or RIP. For inter-routing between different ASes, the mostly practised protocol is Border Gateway Protocol (BGP). 

BGP protocol implies sessions between a border AS router and its peers from other ASes. During BGP session, each AS announces to its peers its own prefixes, plus the routes to other IP prefixes on the network, learned from the other peers. The router running BGP accepts and announces the routes according to BGP policy set by AS administrator. BGP policy also qualifies the decision process on the best route among multiple routes to the same prefix. Once the choice is made, the best route is installed in the Forwarding Information Base (FIB) on the forwarding plane of the router. 

Forwarding Tables - or Forwarding Information Bases (FIBs) - consist of IP prefixes and corresponding next hops. On IP packet arrival, network router uses its forwarding engine to do a lookup into FIB to find the matching prefix for packet's destination IP address and then to forward the packet to the corresponding next hop. In case if there are multiple prefixes matching the same destination IP address, the one with the most number of bits is selected. This prefix is called a ``Longest Prefix Match" (LPM) for the matched IP address. 

The LPM lookup is a potential bottleneck. To avoid queuing delays contemporary routing engines run lookups at the line speed. The constant time lookup is performed at the price of the sophisticated hardware chips called ``Ternary Content Addressable Memory" (TCAM). The entries in FIB are sorted from more to less specific prefixes. Parallel TCAM lookup matches IP address to each entry in FIB, so the top matched entry will be the LPM. 

Different factors, such as the growth of the Internet, traffic engineering and multi-homing add to the superlinear growth of the number of separately announced prefixes. This became a serious concern for network operators working in the Default-Free Zone (DFZ).  Because every TCAM has the limitation on FIB size it can store, the DFZ operators have to upgrade the expensive hardware by analogs with bigger capacities. In addition, hardware-implemented parallel search in TCAM is highly energy-consumptive  and needs more cooling facilities.

\begin{table}[tbp]
	\centering
	\small
	\caption{FIB aggregation process}
	\captionsetup{justification=centering}
	\label{tab:fibentry}
	%	\vspace{0mm}
	\subfloat[Original FIB table]{
		\begin{tabular}{| c | c | c | }
			\hline
			Label & Prefix  & Next hop   \\ \hline
			A & 92.65.0.0/15 & 1    \\ \hline
			B & 92.65.128.0/17 & 1    \\ \hline
			C & 92.65.0.0/17 & 2    \\ \hline
			D & 92.65.64.0 /18 & 3    \\ \hline
			E & 92.65.0.0/19 & 3    \\ \hline
		\end{tabular}
		\label{tab:originalfibentry}
	}
	\\
	\subfloat[Compressed FIB table]{
		\begin{tabular}{| c | c | c | }
			
			\hline
			Label & Prefix  & Next hop   \\ \hline
			F & 92.65.0.0/15 & 1    \\ \hline
			G & 92.65.0.0/17 & 3    \\ \hline
			H & 92.65.32.0/19 & 2    \\ \hline
		\end{tabular}
		\label{tab:filteredfibentry}
	}
	\vspace{-3mm}
\end{table}

Finding solution for routing table scalability problem is particularly important in the context of coming IPv6 era (with address space approximately equal to  $3.4*10^{38}$ possible values).
The long-term solution is to review current network protocols and network architecture. Zhao et al.~\cite{zhao2010routing} describe possible revision of the networking business model in order to compensate expenses of DFZ-operators on upgrading their network operational resources. However, the deployment of such solutions is difficult as it can not be done locally within one AS.

In contrast, FIB compression does not require neither the global deployment nor the operational or hardware expenses. Analysis of the global (FIB\cite{meng2005ipv4},\cite{cidr_report}) shows that about 50\% of BGP-announced prefixes represent the sub-blocks of IP address space, that is also advertised by BGP. Some of this overlapping prefixes may (and most likely) share the same next hop (the number of possible next hops depends on the number of peers that AS has). The most obvious compression can be achieved by eliminating entries with prefixes overlapped by more specific prefixes present in FIB and having the same next hop. On the other hand, entries with more specific prefixes can be eliminated if they share the same next hop with less specific prefixes entries. The examples of such algorithms are Level-1 and Level-2 aggregation.  Algorithms as ORTC~\cite{draves1999constructing} or ORTC-based FIFA~\cite{liu2013fifa} use more sophisticated compression techniques and may reduce FIB by up to 70\%. An example of the original and FIFA-compressed FIB is given on the Table \ref{tab:fibentry}.

Any compression approach must efficiently handle constant next hop updates and prefix removals. The number of such announcements can reach tens of thousand per second during spikes.

We say that the compressed FIB is equivalent to the original FIB, if applying compressed FIB to the router doesn't change router's forwarding behavior: a packet with any possible IP address is forwarded to the same next hop as before FIB compression. Establishing of the equivalence between FIBs is a practical way to avoid misbehavior of the forwarding engine and debug new FIB compression techniques. Given the number of possible 32-bit and 128-bit IP addresses ($2^{32}$ for IPv4  and $2^{128}$ for IPv6 addresses), the brute-force verification of the forwarding equivalence between tables is not realistic.   

\begin{figure}
	\begin{center}
		\includegraphics[clip = true, trim = 2cm 5cm 5cm 1cm, width=.3\linewidth, width=0.4\textwidth]{figures/IMG_TaCo_normalized}
		\caption{\label{fig:taco}Leaf-pushed binary tree for FIB (Table \ref{tab:originalfibentry})}
	\end{center}
	\vspace{-8mm}
\end{figure} 

 % if we have T_1...T_n than we need to run first T_1/T_2 comparison. 2 traversals per each tree. Then if we compare T_2 and T_3, we need to run an additional traversal for T_2 to compare it with T_3. Thus every tree except the first and the last (2 traversals per each tree) one will have to run 3 traversals. 3(n - 2) + 2 + 2 = 3n - 2. 

In this work we present the FIB equivalence verification algorithm with the minimized number of lookups and memory accesses required to run for verifying the equivalence of two or more FIBs. The output of algorithm is either the equivalence statement, or the scopes of IP addresses that will be forwarded differently in the comparable FIBs. We begin with giving the mathematical definition to the problem in Section~\ref{sec:bg}. There, we prove the crucial property of the set of all LPMs of the joint FIB $T$, constructed by adding the entries of the comparable FIBs $T_{1}, T_{2}, ... , T_{n}$ and removing the duplicate entries. The property allows to use the entries of the set of $LPM(T)$ instead of IP addresses, for running next hop comparisons in tables $T_{1}, T_{2}, ... , T_{n}$.

In Section~\ref{sec:design} , we show the implementation of the algorithm based on the properties we proved in the previous section. In the Section~ \ref{sec:evaluation} , we evaluate the algorithm by applying it to the real-world IPv4 and IPv6 routing data from RouteViews Project. In  Section~\ref{sec:related} we discuss the other approaches to solve the FIB equivalence verification problem. In Section~\ref{sec:conclusion} we draw the conclusions on this paper and discuss the possible application of the algorithm and our further steps.

%\begin{figure}
%	\centering
%	\includegraphics
%	\caption{Autonomous Systems and Global Network}
%\end{figure}

==> simulation.tex <==
\section{Emulating an ISP network}
\label{sec:simulation}

The second objective of our work is to set up a \emph{realistic network environment} to demonstrate the performance of our FIB aggregation algorithm.  To this end, we use VirtualBox, BGPSimple, and real ISPs' routing data to emulate a real operational network.  Note that our methodology can be used to emulate any network, but in this section, we use the Internet2 Abilene topology as an example to illustrate our methodology.  

\begin{figure}[tb]
\begin{center}
     \includegraphics[width=2.5in]{figures/topology}
\caption{\label{fig:topology}Virtual Network Setup}
\end{center}
\vspace{-8mm}
\end{figure}

Figure~\ref{fig:topology} shows our virtual network, which includes a total of 9 routers in the Internet2 topology and 9 external BGP speakers belonging to other ISPs that exchange routing information with Internet2.  Each node is on a separate virtual machine.    Each Internet2 router runs either the original Quagga or our updated version of Quagga (specifically the Zebra, OSPF, and BGP daemons).  Each BGP speaker runs the BGPSimple program that sends real routing updates to the BGP peer. 

%TODO: do we run OSPFN on the BGP speaker nodes?
We use OSPF to establish intra-domain connectivity among all of the Internet2 nodes.
%which results in route additions to the Kernel FIB for complete intra-domain connectivity. 
The BGP daemons on each Internet2 node then use this base connectivity to establish BGP peering session with their iBGP peers.  For  simplicity, we use full-mesh iBGP peering, i.e., every router has an iBGP session with every other router in the same network.  For a larger topology, we can use Route Reflectors to reduce the number of iBGP sessions.

In order to attain equivalence between the virtual network and a real world ISP, we need the presence of the huge volume of BGP routing updates in the Internet.  Fortunately, BGP routing table and updates from many ISPs are being collected by a number of projects.  
%This is done through tabledump and update �les which are organized chronologically for a lot of actual internet router pre�xes. These �les include snapshots of routing tables of BGP routers in the internet formatted in the form of route announcements and withdrawals. 
We use the BGP data from the RouterViews project of the University of Oregon~\cite{routeviews} and the BGPMon project of Colorado State University~\cite{BGPmon}. The RouterViews project provides BGP table dumps and update files archived at regular intervals while the BGPMon project provides \emph{live} BGP updates in addition to archived BGP data. 
%These are two among the many freely available data sources which make BGP routing information available and it is possible to use these �les as feeds for BGP speaker applications.

%A real-world routing network transits frequent and consistent volume of network control traf�c in order to maintain end-to-end connectivity between its nodes. The control updates format and handshake mechanisms vary depending on the routing protocol being followed. But these updates, although not constituting the majority of the network traf�c, form a signi�cant part as they control the forwarding information held in the routing tables and thereby the overall routing process. The next section details how we add real-world routing updates to our experimental setup.

%We can make a virtual network equivalent to a real-world routing architecture if we need to simulate a very similar level of control traffic. This requires the infusion and propagation of an equivalent volume of protocol speci�c updates which get processed by the individual routing nodes and cause updates to the routing tables. For the purpose of this paper and our research we will focus the control traf�c speci�c to only the BGP protocol. 

We modified the BGPSimple program to pump the BGP data into the network.  The program first reads a routing table from a BGP table dump file (from RouteViews or BGPMon) and then sends the resulting BGP updates over its BGP session so that the peer can establish an initial BGP table.  Since there are hundreds of thousands of entries in a full routing table, we added pacing to the BGPSimple program  so that the peer does not become overwhelmed by the initial influx of updates.  The program then sends subsequent BGP updates as they become available.  These updates are obtained from either the BGP update files downloaded from RouteViews or a live stream of BGP updates from BGPMon.  
%The BGP speaker can also filter BGP updates based on many parameters such as originating peer and address prefix being advertised. 
%These updates are spoken in the form of BGP announcements and withdrawals which when reach the connected routers, are processed and propagated to other BGP peers in the network. In other words, the BGP feed provided to the speaker in a way determine the control traffic moving around in the network. Therefore to make a node on our virtual network function in a similar to an actual BGP router only required feeding routing updates as processed by latter.
In order to evaluate the performance of our system under high routing load, we used large routing tables with 450,000 prefixes on average. 
%The speakers were also configured to switch over to live BGP update channel of Colorado State once they finish processing their initial tabledump files.



%As each node of the Abilene network represents a separate BGP router having its own volume of peering update channel, we added a total of 9 BGP Speaker nodes (ones speaker for each virtual router node) to our setup. Each of these speakers were con�gured for processing a BGP tabledump �le collected for a recent date from the data sources corresponding to an actual internet BGP router. 

==> stateofart.tex <==
\section{state of the art}
\label{sec:stateart}
Section
